A Survey of Slow Thinking-based Reasoning LLMs using Reinforced Learning and Inference-time Scaling Law

This survey explores recent advancements in reasoning large language models (LLMs) designed to mimic "slow thinking" - a reasoning process inspired by human cognition, as described in Kahneman's Thinking, Fast and Slow. These models, like OpenAI's o1, focus on scaling computational resources dynamically during complex tasks, such as math reasoning, visual reasoning, medical diagnosis, and multi-agent debates. We present the development of reasoning LLMs and list their key technologies. By synthesizing over 100 studies, it charts a path toward LLMs that combine human-like deep thinking with scalable efficiency for reasoning. The review breaks down methods into three categories: (1) test-time scaling dynamically adjusts computation based on task complexity via search and sampling, dynamic verification; (2) reinforced learning refines decision-making through iterative improvement leveraging policy networks, reward models, and self-evolution strategies; and (3) slow-thinking frameworks (e.g., long CoT, hierarchical processes) that structure problem-solving with manageable steps. The survey highlights the challenges and further directions of this domain. Understanding and advancing the reasoning abilities of LLMs is crucial for unlocking their full potential in real-world applications, from scientific discovery to decision support systems.

==> secs/07Disscusion.tex <==
% \input{tabs/method_compare}

% \input{tabs/method_results}

\section{Analysis and Discussion}
\label{Analysis and Discussion}




==> tabs/method_compare.tex <==
% tools:  Symbolic solvers, programs, calculator, No
% CoT: Foundational CoT, Advanced CoT, Long CoT, No
% Training: Pre-training, FT, Prompt
% Access: open \textcolor{green}{\cmark} or close \textcolor{red}{\xmark}
% RL: PPO, DPO, No\textcolor{red}{\xmark}
\begin{table*}[]
% \color{red}
\scriptsize
\caption{\highlight{Comparison of typical mathematical LMs. Pre-T: Pre-Training, FT: Finetuning, MM: Multimodal, Symbolic-S: Symbolic solvers, F-CoT: Foundational CoT, A-CoT: Advanced CoT, RL: Reinforce Learning}}% , M-CoT: Multimodal CoT
\label{table: comparison of mathematical LMs}
\begin{tabular}{lccccccc}
\hlineB{4}
   Methods     & Base Model & Training & Tool & CoT & RL & MM  & Access \\
\hline
GPT-$f$~\cite{polu2020generative}  & - &  Pre-T  & Symbolic-S  & \textcolor{red}{\xmark} & \textcolor{red}{\xmark}  & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\
LISA~\cite{jiang2021lisa}  & -    &   Pre-T   &  Symbolic-S  &  \textcolor{red}{\xmark} & \textcolor{red}{\xmark} &   \textcolor{red}{\xmark}    & \textcolor{red}{\xmark} \\
MATH-PLM~\cite{hendrycks2021measuring} &  GPT-2, GPT-3 &  Pre-T &   \textcolor{red}{\xmark} &  F-CoT &  \textcolor{red}{\xmark}  &  \textcolor{red}{\xmark}  & \textcolor{red}{\xmark} \\
Minerva~\cite{lewkowycz2022solving} & PaLM  &  Pre-T  & \textcolor{red}{\xmark} &  \textcolor{red}{\xmark}  &  \textcolor{red}{\xmark} & \textcolor{red}{\xmark}  & \textcolor{red}{\xmark} \\
MWP-BERT~\cite{liangMWPBERTNumeracyaugmentedPretraining2022} & BERT &  Pre-T  &  \textcolor{red}{\xmark}  &  \textcolor{red}{\xmark}  &  \textcolor{red}{\xmark} & \textcolor{red}{\xmark}  & \textcolor{red}{\xmark} \\
ControlMath~\cite{chen2024controlmath} &  LLaMA-2, Mistral  &  FT   & \textcolor{red}{\xmark} &  F-CoT  &  \textcolor{red}{\xmark}  &  \textcolor{red}{\xmark}  &  \textcolor{red}{\xmark} \\
EURUS~\cite{yuan2024advancing} &  Mistral, CodeLLaMA   &  FT   & \textcolor{red}{\xmark} &  F-CoT   &  DPO, KTO, NCA   &  \textcolor{red}{\xmark}  &  \textcolor{green}{\cmark} \\
MathGLM \cite{yang2023gpt} & GLM  & FT &   \textcolor{red}{\xmark} & \textcolor{red}{\xmark} &  \textcolor{red}{\xmark}  &  \textcolor{red}{\xmark}  & \textcolor{green}{\cmark} \\
WizardLM~\cite{xu_wizardlm_2023}& LLaMA  & FT &    \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{red}{\xmark}  &  \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
Wizardmath~\cite{luo2023wizardmath} & LLaMA-2  &  FT  & \textcolor{red}{\xmark}  & \textcolor{red}{\xmark} & PPO & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
PaLM 2-L-Math~\cite{liu_improving_2023} & PaLM-2-L &  FT & \textcolor{red}{\xmark} &  F-CoT &  \textcolor{red}{\xmark}  & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\
Codex-math~\cite{drori2022neural} & Codex &  Prompt & Program & \textcolor{red}{\xmark} &  \textcolor{red}{\xmark}  & \textcolor{red}{\xmark}  & \textcolor{red}{\xmark} \\
Toolformer~\cite{schick2023toolformer} & GPT-J  &  FT &  Calculator  & \textcolor{red}{\xmark} &  \textcolor{red}{\xmark}  &  \textcolor{red}{\xmark}  & \textcolor{red}{\xmark} \\
LeanReasoner~\cite{jiang2024leanreasoner} & CodeLLaMA &  FT  & Symbolic-S & \textcolor{red}{\xmark} &  \textcolor{red}{\xmark}  & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
LINC~\cite{olausson2023linc} & StarCoder+  &  Prompt  & Symbolic-S  &  F-CoT  & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
MuMath-Code~\cite{yin2024mumath} & Llama-2 &  FT & Program & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} &  \textcolor{green}{\cmark} \\
MAmmoTH~\cite{yue2023mammoth} & - & FT & Program & F-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\
InternLM-Math \cite{ying2024internlmmath} & InternLM2 & Pre-T, FT & Program &  F-CoT & PPO & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
Qwen-Math \cite{yang2024qwen2} & - & Pre-T, FT & Program &  F-CoT & PPO & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
PAL~\cite{gao2023pal} & -  & Prompt & Program & F-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
CoT~\cite{wei2022chain} & -  & Prompt & \textcolor{red}{\xmark} & F-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
PromptPG-CoT~\cite{lu2022dynamic} & - & Prompt & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
BoostedPrompt~\cite{pitis_boosted_2023} & - & Prompt & \textcolor{red}{\xmark} & F-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{red}{\xmark}\\
ToT~\cite{yao2023tree} & - & Prompt & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} &  \textcolor{green}{\cmark} \\
PoT~\cite{chen2022program} & - & Prompt & Program &  F-CoT & \textcolor{red}{\xmark}  & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
Self-check~\cite{miao2023selfcheck} & - & Prompt & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
Self-Consistency~\cite{wang2022self}& - & Prompt & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
Diversity-of-Thought~\cite{naik2023diversity}& - & Prompt & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\
RAP~\cite{hao2023reasoning} &  - & Prompt & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
LATS~\cite{zhou2023language} &  - & Prompt & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\
LLM+P~\cite{liu2023llm+} & - & Prompt &  Symbolic-S & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
LLM+DP~\cite{dagan2023dynamic} & - & Prompt &  Symbolic-S & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
ISR-LLM~\cite{zhou2023isr} &  - & Prompt & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
MCR~\cite{yoran2023answering} & - & Prompt & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
Rank-verifier~\cite{cobbe2021training} &  - & Prompt & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\
GRACE~\cite{khalifa2023discriminator} & - & Prompt & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
Reflexion~\cite{shinn2023reflexion} & - & Prompt & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
CR~\cite{zhang2023cumulative} & - & Prompt & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
Step-Plan~\cite{zhang2023interpretable} & - & Prompt & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
STaR~\cite{zelikman2022star}& GPT-J & FT & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
V-STaR~\cite{hosseini2024v}& LLaMA2, CodeLLaMA & FT & \textcolor{red}{\xmark} & A-CoT & DPO &  \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\
Quiet-STaR~\cite{zelikman2024quiet}& Mistral & Pre-T & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} &  \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\
REFT~\cite{luong2024reft} &  Galactica, CodeLLaMA  & FT &  \textcolor{red}{\xmark}  & A-CoT &  PPO  & \textcolor{red}{\xmark} &  \textcolor{green}{\cmark} \\
SCoRe~\cite{kumar2024training}& Gemini & FT & \textcolor{red}{\xmark} & A-CoT  & SCoRe &  \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\
HGS-PRM~\cite{ma2023let}& LLaMA2, WizardMath & FT & \textcolor{red}{\xmark} & A-CoT & PPO &  \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\
MCTSr~\cite{zhang2024accessing}& LLaMa-3 & FT & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} &  \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
CoRe~\cite{zhu2022solving}& GPT-J, DeBERTa-large & FT  &  \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} &  \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
Marco-o1~\cite{zhao2024marco}& Qwen2 &  FT & \textcolor{red}{\xmark} & A-CoT  & \textcolor{red}{\xmark} &  \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
Step-DPO~\cite{lai2024step}& Qwen2 &  FT  & \textcolor{red}{\xmark} & A-CoT & DPO &  \textcolor{red}{\xmark} &  \textcolor{green}{\cmark} \\
Flow-DPO~\cite{deng2024flow}& LLaMA3, Phi-3  & FT &  \textcolor{red}{\xmark} & A-CoT & DPO &  \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\
OmegaPRM~\cite{luo2024improve}&  Gemini Pro, Gemma2 & FT  & \textcolor{red}{\xmark} & A-CoT & PRM &  \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\
% SocratiQ~\cite{al2023socratic}&  &   &  & &  &  \textcolor{red}{\xmark} &  \\
SocraticLLM~\cite{ding2024boosting}& Qwen2 &  FT  & \textcolor{red}{\xmark} & A-CoT & \textcolor{red}{\xmark} &  \textcolor{red}{\xmark} &  \textcolor{green}{\cmark}\\
MATHDIAL~\cite{macina2023mathdial}& T5 &  FT & \textcolor{red}{\xmark} &  A-CoT & \textcolor{red}{\xmark} &  \textcolor{red}{\xmark} & \textcolor{green}{\cmark} \\
QwQ \cite{qwq-32b-preview}& Qwen2.5 &  Pre-T  & \textcolor{red}{\xmark} & Long CoT & \textcolor{green}{\cmark} &  \textcolor{red}{\xmark} &  \textcolor{green}{\cmark} \\
o1 \cite{openai_o1_system_card}  &  - &   Pre-T   &   \textcolor{red}{\xmark} &  Long CoT   &  \textcolor{green}{\cmark}  & \textcolor{green}{\cmark} & \textcolor{red}{\xmark} \\
GPT-4o~\cite{hurst2024gpt}& - & Pre-T  & \textcolor{green}{\cmark} & A-CoT & \textcolor{green}{\cmark} &  \textcolor{green}{\cmark} & \textcolor{red}{\xmark} \\
GPT-4V~\cite{openai2023gpt4}& - & Pre-T  & \textcolor{green}{\cmark}  & A-CoT & \textcolor{green}{\cmark} &  \textcolor{green}{\cmark} &  \textcolor{red}{\xmark}\\
Qwen2-VL~\cite{Qwen2-VL}& Qwen2-VL & Pre-T  & \textcolor{red}{\xmark} & F-CoT & \textcolor{red}{\xmark} &  \textcolor{green}{\cmark} & \textcolor{green}{\cmark} \\
LLaVA-o1~\cite{xu2024llava}&  LLaVA&  FT & \textcolor{red}{\xmark} & Long CoT & \textcolor{red}{\xmark}  &  \textcolor{green}{\cmark} & \textcolor{green}{\cmark} \\
Gemini~\cite{team2023gemini}& Gemini &  Pre-T & \textcolor{green}{\cmark} &  A-CoT & \textcolor{green}{\cmark} &  \textcolor{green}{\cmark} & \textcolor{red}{\xmark} \\
GLM-4V~\cite{glm2024chatglm}& ChatGLM &  Pre-T  & \textcolor{green}{\cmark} & A-CoT & \textcolor{green}{\cmark} &  \textcolor{green}{\cmark} & \textcolor{red}{\xmark} \\
AtomThink~\cite{xiang2024atomthink}& LLaVA, EMOVA & FT  & \textcolor{red}{\xmark} & Long CoT  & PRM  &  \textcolor{green}{\cmark} & \textcolor{green}{\cmark} \\
Math-LLaVA~\cite{shihu2024mathllava}& LLaVA & FT  & \textcolor{red}{\xmark} & F-CoT  &  \textcolor{red}{\xmark} &  \textcolor{green}{\cmark} &  \textcolor{green}{\cmark} \\
M-STAR~\cite{anonymous2024diving}& MiniCPM-V & FT  & \textcolor{red}{\xmark} & A-CoT & PRM &  \textcolor{green}{\cmark} & \textcolor{red}{\xmark} \\
UnAC~\cite{wang2024understanding}& GPT-4V, Gemini, LLaVA &  Prompt & \textcolor{red}{\xmark} & F-CoT & \textcolor{red}{\xmark}  &  \textcolor{green}{\textcolor{green}{\cmark}} & \textcolor{red}{\xmark}  \\
\hlineB{4}
\end{tabular}
\end{table*}




==> tabs/summary_of_RL.tex <==
\begin{table*}[t!]
\centering
\small
\caption{summary of RL}
\label{table: RL Algorithm}
\setlength{\tabcolsep}{1.6mm}{
\resizebox{\linewidth}{!}{
\begin{tabular}{lll >{\raggedright\arraybackslash}m{0.5\textwidth}}
\hline
% Category是online RL(在线) 和 offline RL（离线）

Algorithm & paper &  Category & Characteristic \\
\hline
DPO  & \cite{rafailov2024direct} & offline &  The proposed strategy is directly optimized utilizing preference data, thereby eliminating the necessity for reward modeling. Model training is accomplished through systematic comparative analysis of the relative quality of different responses.\\


PPO & \cite{schulman2017proximal}  & online  & The proposed strategy is directly optimized by maximizing expected rewards via policy gradient methods. \par
To ensure algorithmic stability, pruning constraints are systematically incorporated into the policy update phase.
 \\

 
GRPO & \cite{shao2024deepseekmath} & online & Building upon the PPO algorithm, we have made improvements by eliminating the value function. Instead, we estimate advantages by collecting multiple outputs for the same question, thereby streamlining and accelerating the RLHF training process. \\


Rule-reward & \cite{bignold2023persistent}   & offline & Output quality is evaluated through predefined rules, such as verifying whether responses adhere to predefined formatting guidelines or logical coherence.\\


CPPO & \cite{lin2025cppo} & online & 
GRPO is accelerated by accomplishing pruning, retaining only completion results with high absolute advantage for gradient updates. Additionally, a dynamic allocation strategy for completion results is introduced to fully utilize GPU resources.
\\


RLOO & \cite{ahmadian2024back} & online & The strategy is continuously updated through online interaction, characterized by high real-time performance, thereby enabling rapid adaptation to environmental changes.
\\


PRIME & \cite{cui2025process} & online &Process reinforcement is accomplished via implicit rewards, aimed at enhancing the reasoning abilities of language models. This approach eliminates the need for explicit process labels, thereby providing implicit process rewards.\\
\hline
\end{tabular}
}
}
\end{table*}

==> tabs/summary_of_Reward_design.tex <==
\begin{table*}[t!]
\centering
\small
\caption{summary of Reward designs}
\label{table: Reward designs}
\setlength{\tabcolsep}{1.6mm}{
\resizebox{\linewidth}{!}{
\begin{tabular}{lllllll}
\hline
%data source 有 data construction ,sampling,human annotation
% RL是强化算法：DPO,PPO,GRPO,RLOO,PRIME
% learning 是微调方法：RL,SFT,COT

Category & paper & Data Source& RL & learning    \\ 
\hline
ORM  & DeepSeek-R1 &        &   TasksMultiple  & GPRO  &  RL\&SFT \\
     &  &        &         &      &    &\\


\hline
PRM & \\






\hline
\end{tabular}
}
}
\end{table*}
